Closed-form congestion control via deep symbolic regression

As mobile networks embrace the 5G era, the interest in adopting Reinforcement Learning (RL) algorithms to handle challenges in ultra-low-latency and high throughput scenarios increases. Simultaneously, the advent of packetized fronthaul networks imposes demanding requirements that traditional congestion control mechanisms cannot accomplish, highlighting the potential of RL-based congestion control algorithms. Although learning RL policies optimized for satisfying the stringent fronthaul requirements is feasible, the adoption of neural network models in real deployments still poses some challenges regarding real-time inference and interpretability. This paper proposes a methodology to deal with such challenges while maintaining the performance and generalization capabilities provided by a baseline RL policy. The method consists of (1) training a congestion control policy specialized in fronthaul-like networks via reinforcement learning, (2) collecting state-action experiences from the baseline, and (3) performing deep symbolic regression on the collected dataset. The proposed process overcomes the challenges related to inference-time limitations through closed-form expressions that approximate the baseline performance (link utilization, delay, and fairness) and which can be directly implemented in any programming language. Finally, we analyze the inner workings of the closed-form expressions.

==> sections/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bios/jeanMartins.jpg}}]{Jean
P. Martins} received his Ph.D on Computer Science from the ICMC at the University of São Paulo
(2015) and his masters from the Federal University of Goiás (2010). He was also a post-doc
researcher at University of Coimbra (2016). Since 2018 he works as an Experienced Researcher in
Artificial Intelligence at Ericsson Research. His main research interests intersect combinatorial
optimization, evolutionary algorithms, multi-agent systems and deep reinforcement learning.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bios/IgorAlmeida.png}}]{Igor
Almeida} received in 2010 a B.Sc. degree in computer engineering, and in 2013 an M.Sc. degree in
electrical engineering, both from the Federal University of Pará (UFPA), Belém, Brazil, where he is
currently pursuing a Ph.D. degree in electrical engineering. He has been with Ericsson Research
since 2016, involved with topics such as 5G, fronthaul networking, synchronization and wireless
communications. \end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,
clip]{bios/bio_ricardo_souza.png}}]{Ricardo Souza} received his B.Sc. degree in electrical
engineering from the Federal University of Campina Grande (UFCG) in 2008 and in 2011 his M.Sc. in
computer engineering from University of Campinas (Unicamp) where he is currently pursuing a Ph.D.
degree. Since 2016 he works as an Artificial Intelligence Researcher at Ericsson Research Brazil.
His research interests include distributed systems, multi-agent systems, deep reinforcement learning
and networked robotics.  \end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{bios/SilviaLins.jpg}}]{Silvia
Lins} is an Experienced Researcher from the Networks area at Ericsson Research Brazil. She received
her B. Sc. degree in Computer Engineering from the Federal University of Pará (UFPA) in 2011 and her
M.S. on Electrical Engineering in 2013 from the same university, where she is also doing her Ph.D.
Currently her work focuses on machine learning for transport and mobile networks optimization.
\end{IEEEbiography}

